Scalable Real-time Transport of Baseband Traffic

In wireless deployments, such as Massive-MIMO, where radio front-ends and back-end processing are connected through a transport network, meeting the real-time processing requirements is essential to realize the capacity gains from network scaling. While simple forms of baseband transport have been implemented, their real-time analysis at much larger scale is lacking. Towards this, we present the design, delay, and capacity analysis of baseband transport networks, utilizing results from real-time systems in the context of wireless processing. We propose a novel Fat-Tree-based design, called DISTRO, for baseband transport, which is a real-time network that bounds the maximum end-to-end transport delay of each baseband packet. It achieves this by placing design constraints and bounding the queuing delay at each aggregation point in the network. We further characterize the wireless capacity using DISTRO and provide an efficient search algorithm for the design of a capacity achieving baseband transport.

==> all.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Background %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \subsection{Possible Topologies}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Architecture %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{DISTRO: Scalable Real-Time Transport Design}\label{architecture}

In this section, we present \algnameD, a real-time transport design for
baseband traffic that is scalable across radios. \algnameD's architecture
enables real-time baseband transport and provides end-to-end schedulability.

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/tree_main_1}
    \caption{Fat-Tree architecture of DISTRO with heterogeneous radios.\label{fig:tree_main}}
\end{figure}

\subsection{Design Philosophy}

As the baseband network is a dedicated network, its design can assume
a centralized view where the information about the entire network, its topology,
and traffic, is available. The traffic flow is exclusively between the radios and the
processor pool with no cross-traffic between radios. Further, the network should address
the practical constraints such as a limited number of ports per switch, flexible
radio selection, and fault-tolerance. \algnameD is designed keeping in mind the
following requirements:

\begin{itemize}
\item Guarantees: The baseband transport must operate in real-time and provide
guarantees on delivery. Specifically, given the traffic flows and delay bounds,
we must be able to give a sufficient, if not necessary, condition to check their
end-to-end schedulability.

\item Scalability: The network must accommodate an increasing number of radios
without severely affecting their delay performance, and its schedulability must
be flexible to addition and removal of radios.
\end{itemize}
%

% centralized design, info about all radios is available
% eliminate queuing at core network
\noindent Fig.~\ref{fig:tree_main} shows the deployment of \algnameD with a \emph{Fat-Tree}
structure. The radios are connected to edge switches, and the links from the edge
switches are aggregated at multiple levels till the root switch. The destination
point is assumed to be located at the root switch, which is the common aggregation point
for the baseband packets. The destination could be either a physical or a virtual
point that is connected to a pool of baseband processors.

The network has two components: edge switches and aggregation network.
The edge switches are the first entry point of every baseband
flow. Each edge switch connects a group of radios that are in physical proximity,
for instance, a cellular site. The aggregation network consists of all remaining
switches except the edge switches, and its purpose is to aggregate
traffic from edge.


\subsection{Symmetric Fat-Tree Architecture}

The aggregation network in \algnameD is a logical tree of links and switches. In
particular, it is a Fat-Tree which is defined as follows.

\begin{definition}
A tree is a Fat-Tree if for every switch in the tree the switch's uplink
capacity is greater than or equal to the sum capacity of the incoming links.
\end{definition}
%
\noindent While Fat-Tree deployments were also proposed in data-center networks \cite{alfaras},
they are a natural choice for baseband transport where centralization is an important
requirement. Furthermore, a tree structure is inherently scalable where few switches
can connect a large number of radios. Also, the aggregation tree in \algnameD is
assumed to be symmetric where the following definition holds:

\begin{definition}
A tree is symmetric if for every switch, interchanging the incoming links yields the
same tree.
\end{definition}
%
\noindent From the symmetry property, the aggregation tree is necessarily a full
tree.  Fig.~\ref{fig:tree_main} shows an aggregation tree where three
switches are connected to the root switch through a 20G link. Clearly, it is a
symmetric tree as its mirror image yields the same tree.
% an aggregation tree is applicable in general to any $q$-ary tree
% with $q$ incoming links per switch.


\subsection{End-to-End Guarantees}\label{sec:guarantees}

We characterize the schedulability of baseband traffic in our network. As noted
earlier, a packet can experience a queuing delay at any of the switches in the network.
Beyond the edge switch, characterizing the queuing behavior becomes difficult as
the packet arrivals are no longer periodic \cite{hui:95}. However, under our
symmetric Fat-Tree construction, one can readily obtain the bound on the waiting time.

Assume $K$ edge switches, and let $S_i, i = 1,2, \ldots K$, denote the set of
radios connected to edge switch $k$ where $S_k \subseteq \{1,2 \ldots, n\}$.
For simplicity, assume at time $t=0$ packets from radios of each edge switch
are queued at the switch, and the packets arrive periodically at the switch
thereafter. Further assume no transmission or propagation delay from the radio to
the edge switch. Let $C_1$ denote the transmission time of a packet on the link
connecting the edge switch and the next aggregation switch. Since packet size, $B$,
is fixed for the network, every baseband packet has the same transmission time
going through the edge switch.


\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/path}
    \caption{Path of baseband packet from the source to destination.\label{fig:path}}
\end{figure}


\begin{figure}
    \centering
    \subfigure[Equal transmission times]{\label{fig:equal}\includegraphics[width=0.35\columnwidth]{figures/unblocking}}
    \hspace{8mm}
    \subfigure[Unequal transmission times]{\label{fig:unequal}\includegraphics[width=0.35\columnwidth]{figures/blocking}}
    % \vspace{-10pt}
    \caption{Blocking of $c$ by at most one packet (left) and more than one packet (right).\label{fig:blocking}}
\end{figure}



For simplicity, assume a binary aggregation tree. Let the
transmission time sequence as a packet traverses from the edge to the destination be
represented as $C_1, C_2, \ldots, C_{h+1}$, where $h$ is the height of the aggregation
tree. We define $h=1$ if there is only one aggregation switch.

From the symmetric Fat-Tree definition, it holds that if $C_j$ is the transmission
time on the incoming link, then the transmission time on the aggregation link, $C_{j+1}$,
for all $j, 1 \leq j \leq h$, satisfies:
\begin{equation}
 C_{j+1} \leq C_{j}/2 \label{eq:fatness}
\end{equation}
%
Let us assume the edge-switch uses a non-preemptive scheduling policy while the
aggregation switches use FIFO scheduling. Under non-preemptive scheduling,
the inter-arrival time of the incoming packets from the edge is equal to or
larger than $C_1$. Consider the first aggregation switch: the outgoing
transmission time is $C_2 (C_2 \leq C_1/2)$. The packets in each of the two incoming
links have at least $C_1$ time separation. Therefore, any packet will wait for
at most $C_2$ time in the queue, which occurs when two packets arrive at the same
time. This is illustrated in Fig.~\ref{fig:equal}, where packet $c$ arrives at the
same instant as packet $b$, and is blocked by the transmission time of packet $b$.

In a similar manner, for every $j$, packets in the two incoming links
with transmission time $C_j$ and inter-arrival time greater than $C_j$, will have
a maximum queuing delay of $C_{j+1}$. Therefore, for the path as shown in
Fig.~\ref{fig:path}, the maximum total delay of \emph{any} baseband packet across the
aggregation network is bounded by:
\begin{eqnarray}
T_a = \sum_{j=2}^{h+1} ( t_s + C_{j} + C_{j} + t_p) &=& h(t_s + t_p) + \sum_{j=2}^{h+1} 2C_{j}\\
&\leq& h(t_s + t_p) + \sum_{j=2}^{h+1} \frac{C_1}{2^{j-2}} \\
&=&  h(t_s + t_p) + 2(1-2^{-h})C_1 \label{eq:max_delay}
\end{eqnarray}
%
where we use the inequality, $C_j \leq C_{j-1}/2\leq \ldots \leq C_{1}/2^{j-1}$, using
Eq.\eqref{eq:fatness}.

Now, in order for a baseband packet of radio $i$ to meet its end-to-end delay bound
$D_i$, the total packet delay at its edge switch must be less than $D_i$ less the
maximum aggregation delay. Adding the switching and propagation delay of the
edge switch, we arrive at the end-to-end schedulability of all baseband flows in
the network by checking the schedulability of baseband traffic at each edge switch.
%
\begin{theorem}\label{theorem:distro}
In a $q$-ary symmetric fat-aggregation-tree of height $h$, the radio traffic $\tau_i = (T_i, D_i), i = 1,2,\ldots, n$,
is schedulable, if for every $k, 1 \leq k \leq K$, the set of traffic flows
$\tau_i = (T_i, d_i^{'}), i \in S_k$, with transmission time $C_1$ and no preemption,
is schedulable at edge switch $k$, where $d_i' = D_i - \frac{1-q^{-h}}{1-q^{-1}}C_1 - (h+1)(t_s + t_p)$.
\end{theorem}
%
\begin{proof}\let\qed\relax
By extension of the binary tree analysis to $q$-ary tree. The maximum queuing delay
of packet on a link with transmission time $C_j$ is $(q-1)C_j$. \qedwhite
\end{proof}
%
\noindent Theorem \ref{theorem:distro} provides only a sufficient condition for schedulability,
but does not affirmatively tell us if a given set of traffic flows are schedulable.
Nevertheless, the result is still useful as it allows us to construct a transport network
that guarantees to meet the requested end-to-end delay bounds. Furthermore, it
gives the scheduling policies that the network must implement: non-preemptive
scheduling at edge-switch, and regular FIFO scheduling at aggregation switches.

The reason we restrict our construction to a symmetric Fat-Tree and non-preemptive
scheduling is simple: the packet transmission times are equal for the incoming links,
and therefore, the maximum queuing delay in the aggregation network is easy
to obtain. This is not the case, however, if we assume unequal transmission times,
which happens if unequal links are used or when preemption is allowed. For instance,
Fig.~\ref{fig:unequal} shows the blocking of a smaller packet, $c$, due to the
transmission of two previous larger packets. This example is akin to the head-of-line (HOL)
blocking problem that occurs when subsequent transmissions are held up by the first
transmission \cite{hol}. Then, to arrive at the maximum queuing time in the network,
one must examine different arrival sequences and their transmission times at each
switch, which can quickly become intractable.



\subsection{Scalability}

% two-types: delay is logarithmic, schedulability is local at edge switch
The design of \algnameD is scalable on three fronts. First, as the number of
radios in the network, $n$, grows, and the number of edge switches, $K$ increases,
the maximum total delay of a packet increases only logarithmically. To see this,
one can write the upper bound on Eq.\eqref{eq:max_delay} as follows:
%
\begin{equation}
T_a < h(t_s + t_p) + 2C_1
\end{equation}
%
The delay bound grows linearly with the height, $h$, which is always less than
or equal to $\lceil \log_2 K\rceil$. For large packets (e.g. Jumbo Ethernet frames),
the transmission time is much larger than the switching and propagation time. In
this case, the delay scaling factor, $t_s+t_p$, becomes even less significant.

Second, \algnameD supports heterogeneous baseband radios with differing periods
and deadlines. There is no restriction on the type of radio protocol. This aids
the deployment of a radio-access network (RAN) over multiple wireless standards,
such as LTE and WiFi, in the same physical location.


Finally, each edge switch, $k$, implements a schedulability test locally that is
dependent only on the traffic generated from the  set of radios, $S_k$, connected
to it. Any addition or removal of radios requires one to check only local schedulability,
without disturbing the performance of other flows. This is a nice property to have
since in practice the network deployment is incremental.

% Since most modern switches support tens of ports, the typical height of the
% aggregation tree will quite small in practice. One

\subsection{Run-time Scheduling}

The aggregation network in \algnameD implements the default FIFO scheduling. On
the other hand, each edge switch implements a non-preemptive scheduler which can
either be EDF or fixed-priority. The fixed-priority scheduler is easy to realize
with multiple outbound queues at a switch. Each incoming packet is first classified
and placed in its corresponding queue, and the queues are then dequeued in order
of their priority.

\emph{Background Traffic}. Background traffic such as control messages can disrupt
the real-time performance of the network. To ensure minimum disruption, we
segregate the baseband traffic from the rest of the traffic through flow
prioritization. Background and rest of the traffic are placed in a separate queue,
which has lower priority than baseband traffic. Since background traffic
adds to the non-preemptive delay at each switch, we update the delay bound in
Eq.\eqref{eq:max_delay} accordingly.


\section{Evaluation}\label{evaluation}

We implement and evaluate \algnameD's Fat-Tree architecture using NS-3\cite{ns3}.
NS--3 is a discrete-event network simulator that accurately simulates network
traffic in large deployments. Table~\ref{table:simu_params} shows the simulation
parameters used in our setup. Each edge switch connects 4 heterogeneous radios that
have different flow rates (1,1.5,2 and 2.5G) but fixed packet size of 1000 Bytes.
We simulate a fat-aggregation-tree with three levels: 1) a core switch that is connected
to the destination through 200 Gbps link; 2) $q$ aggregation switches connected to
core switch with 40Gbps links; 3) $q$ edge switches connected to each aggregation
switch with 10Gbps links. Thus, the total number of radios in our setup is $4q^2$.

\begin{table}
\centering
\small{
    \begin{tabular}{|c|c||c|c|}
    \hline
    $t_s$ & 50ns &  Edge--src.   & 10Gbps   \\
    \hline
    $t_p$  & 10ns  & Agg.--Edge & 10Gbps   \\
    \hline
    Pkt. size ($B$) & 1KB & Agg.--Core & 40Gbps \\
    \hline
    $q$-ary tree & 2,3,4  & Core--Dest.  & 200Gbps\\
    \hline
    height ($h$) &  2  & Flow rate ($R_i$) & 1, 1.5, 2, 2.5 Gbps\\
    \hline
    Radios/edge & 4  & Simulation Time & 1sec\\
    \hline
    \end{tabular}
    }
\caption{Simulation parameters}
\label{table:simu_params}
% \vspace{-15pt}
\end{table}
%
%
% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\columnwidth]{figures/radio_delays_3}
%     \caption{Maximum transport delay and jitter of each flow in a 36--radio setup. \algnameD
%     meets the end-to-end guarantees of all flows.\label{fig:radio_delays_3}}
% \end{figure}
% %
%
\begin{figure}
    \centering
    \subfigure[Maximum Delay]{\includegraphics[width=0.75\columnwidth]{figures/radio_delays_3}}
    \vspace{1mm}
    \subfigure[Jitter]{\includegraphics[width=0.75\columnwidth]{figures/radio_jitters_3}}
    % \vspace{-10pt}
    \caption{Delay metrics for flows in a 36--radio setup. \algnameD
    meets the end-to-end guarantees of all flows.\label{fig:radio_delays_3}}
\end{figure}
%

We use the NS--3 packet tagging mechanism to tag each baseband packet with a
priority level. The priority levels are chosen to achieve end-to-end schedulability
(Sec.~\ref{sec:guarantees}). We then implement a packet-classifier at the edge switch
that classifies the incoming packet and places it in one of the 4 egress queues. For
dequeuing, the queues are searched in decreasing order of their priority.


Fig.~\ref{fig:radio_delays_3} shows the maximum end-to-end transport delays and
jitter observed in a 3-$ary$ tree with 36 radios. Here, we compare \algnameD's scheduling with the basic
FIFO packet scheduling. For simplicity, we assume the transport delay-bound is same
as the inter-arrival period of each flow. Under this assumption, the priorities
are determined by the inverse to the period (equivalent to a rate-monotonic scheduler).
\algnameD meets the end-to-end guarantees of each flow while the FIFO scheduling misses
the delay bound of the 2.5G flow. In prioritized scheduling, the 1G flow has the
least priority and therefore sees an increase in its transport delay.

%
\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/scale_delay}
    \caption{Maximum end-to-end delay of flows with increasing number of radios.\label{fig:scale_delay}}
\end{figure}
%

In Fig.~\ref{fig:scale_delay}, we show the maximum observed flow delays as we increase
the number of radios in the network. Assuming a fixed number of radios per
edge switch, the scaling is achieved by using $q^2$ edge switches, and $q$ aggregation
switches for a $q$-ary aggregation tree. The core switch capacity, however, is
fixed at 200Gbps. Despite quadrupling the number of radios (from 16 to 64),
the maximum delay in the network increases not more than $300$ns (less than 10\%
increase). This is attributed to the maximum delay bound that is dependent only
on the height of the tree, and not on the number of radios. Note that this
constant increase is not always the case, for example, in daisy-chained radio
network in ARGOS\cite{argos}, the maximum delay grows linearly with the number
of radios.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% rate %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Capacity with Scheduling}\label{application}


In this section, we characterize the achievable MIMO capacity under the practical
constraints of deadlines. The system requests a transport delay bound for each
baseband packet, and packets that are delayed more than their delay bound are
discarded. Decoding is considered successful only if for every radio the maximum
transport delay of its baseband packets is less than its delay bound. We wish to
find the packet scheduling policy that maximizes the system capacity.


%
\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/radio_model}
    \caption{System model for MIMO decoding.\label{fig:radio_model}}
\end{figure}
%


Consider the system model shown in Fig.~\ref{fig:radio_model}, Let $\ve{x} \in \mathbb{C}^{m\times 1}$
be the signal vector sent by the transmitter, and let $\ve{y} = \mathbb{C}^{n\times 1}$
be the received signal vector, where $m$ is the number of transmit antennas, and $n$
is number of radios. Let $\ve{H} \in \mathbb{C}^{n\times m}$ be the channel matrix
between the transmitter and the radios.

\textbf{Transport}. Assume fixed packet size $B$, and let $L$ denote the aggregation
capacity of the switch. Since we are interested in the queuing delays, we ignore the transmission
time from radio to the switch, the propagation, and the switching delays. From
Eq.~\eqref{eq:distro:arrival}, the inter-arrival time at radio $i$ is $T_i = \frac{B}{2Q_if_i}$.

\textbf{ADC Quantization}. Let us assume radio $i$ has ADC quantization width,
$Q_i$, that takes an integer value between $Q_l$ and $Q_h$ bits, where $Q_l$ and $Q_h$
are the minimum and the maximum quantization widths respectively. Further, define
$\ve{Q} = [Q_1, \ldots, Q_n]$, and let $\gamma(Q_i)$ be the average quantization
noise power injected into the baseband samples where $\gamma(\cdot)$ is the quantization
noise function.

Assuming perfect synchronization and a
narrowband channel, the received signal can be expressed as:
%
\begin{equation}\label{eq:sig_mimo}
\ve{y} = \ve{H}\ve{x} + \ve{z} + \ve{z}_Q
\end{equation}
%
where $E[\ve{x} \ve{x}^H] = \rho \ve{I}_{m}$ and $\rho$ denotes the transmitted power,
and $\ve{z} \sim \mathcal{C}\mathcal{N}(0,\sigma^2\ve{I}_{n})$ is the additive complex white gaussian noise, and
$\ve{z}_Q$ represents the quantization noise vector. We assume the effect of quantization manifests through
the an additive term, $\ve{z}_{Q}$, which is approximated as zero-mean complex gaussian noise with covariance
matrix $\ve{\Sigma}_Q = \text{diag}(\gamma(Q_i), \ldots, \gamma(Q_n))$. Further define
$\ve{\Sigma} = \sigma^2\ve{I}_{n} + \ve{\Sigma}_Q$.

% \subsection{Decoding}

% Assume that perfect channel state information is available at the receiver through
% the use of training sequences. Using a Zero-forcing detector \cite{varanasi}, the
% estimated symbol vector is given by:
% %
% \begin{align}
% \hat{\ve{x}} = \ve{x} + (\ve{H}^H \ve{\Sigma}^{-1} \ve{H})^{-1}\ve{H}^H \ve{\Sigma}^{-1}(\ve{z} + \ve{z}_{Q})
% \end{align}
% %
% where $\ve{\Sigma} = \ve{I}_{n} + \ve{\Sigma}_Q$. The SNR of symbol stream $j, 1\leq j \leq m$,
% is:
% %
% \begin{align}
% \gamma_j = \frac{\rho}{[(\ve{H}^H \ve{\Sigma}^{-1}\ve{H})^{-1}]_{j,j}}
% \end{align}
% %
% where $\ve{A}_{i,i}$ denotes the $i$th diagonal element of a square matrix $\ve{A}$. The
% corresponding achievable sum rate (in bits/s/Hz) averaged over different channel realizations is:
% %
% \begin{align}
% R(\ve{Q}) = \mathbb{E}_{\ve{H}} [\sum_{j=1}^{m} \log_2(1 + \gamma_j)]
% \end{align}
% %
% % \begin{theorem}
% Constraining the quantization to ensure the end-to-end schedulability, the maximum
% wireless rate of a system with $n$ radios with deadlines is given by:
% %
% \begin{equation}\label{eq:cap_mimo}
% \max_{\ve{Q} \in [Q_{l}, Q_h]^{n}} R(\ve{Q})\\
% \end{equation}
% %
% such that traffic flows $\tau_i = (T_i, D_i), i \in \{1,\ldots,n\}$, with transmission time
% $B/L$ are schedulable, where $D_i$ is the transport delay bound of radio $i, i \in \{1, \ldots, n\}$.

% As the quantization widths are discrete values, the optimization problem can be
% solved through iterative search of $Q_i$ that satisfy schedulability and achieve
% the maximum rate.

\textbf{Capacity}. The achievable wireless capacity for a fixed $\ve{Q}$ and given
channel $\ve{H}$ is:
%
\begin{align}
R(\ve{Q}) = \log_2 \text{det} (\ve{I} + \ve{\Sigma}^{-1}\ve{H}\ve{H}^{H})
\end{align}
%
Constraining the quantization to ensure the end-to-end schedulability, the maximum
wireless capacity of a system with $n$ radios with deadlines is given by:
%
\begin{equation}\label{eq:cap_mimo}
\text{OPT:} \quad \max_{\ve{Q} \in [Q_{l}, Q_h]^{n}} R(\ve{Q})
\end{equation}
%
such that traffic flows $\tau_i = (T_i, D_i), i \in \{1,\ldots,n\}$, with transmission
time $B/L$ are schedulable, where $D_i$ is the transport delay bound of radio
$i, i \in \{1, \ldots, n\}$.


\begin{prop}
If $\gamma(\cdot)$ is monotonically decreasing, $R(\ve{Q})$ is monotonically increasing in $\ve{Q}$.
\end{prop}

\begin{proof}
Let $\lambda_1, \ldots, \lambda_n$ be the eigen values of $\ve{H}\ve{H}^{H}$. We note
that the eigen values of the linear transformation $\ve{Z}\ve{H}\ve{H}^{H}$ are $r_1\lambda_1, \ldots, r_n\lambda_n$
if $\ve{Z} = \text{diag}(r_1, \ldots, r_n)$ is a non-singular diagonal matrix. Therefore, we can
write $\text{det} (\ve{I} + \ve{\Sigma}^{-1}\ve{H}\ve{H}^{H}) = \Pi_{i=1}^{n}(1 + \lambda_i/(\sigma^2+\gamma(Q_i)))$,
and since $\log()$ is a monotonic transformation, $R(\ve{Q})$ strictly increases if $\gamma(Q_i)$ strictly
decreases with $Q_i$ for any $i$.
\end{proof}


\begin{prop}
If $\tau_i = (T_i, D_i), i \in \{1,\ldots,n\}$ with quantization $\ve{Q}$ are schedulable
with the sufficient conditions of scheduling in Theorem \ref{theorem:fixed}--\ref{theorem:edf},
they remain schedulable by decreasing $\ve{Q}$.
\end{prop}

\begin{proof}
For simplicity, we consider a non-preemptive EDF scheduler and show that the property holds.
For any $i$, changing $Q_i$ to $Q_{i}^{'}$ increases the inter-arrival period from
$T_i$ to $T_i^{'}$. Using the fact that $\lceil{(t-d_i)/T_i^{'}}\rceil^{+} \leq \lceil{(t-d_i)/T_i}\rceil^{+}$,
and substituting in Eq.~\eqref{eq:edf}, it follows that $\tau_i = (T_i^{'}, D_i)$, $i \in \{1,\ldots,n\}$
are schedulable.
\end{proof}

% \begin{prop}
% If $\ve{Q}^\star$ is a solution, then any permutation $\pi(\ve{Q}^\star)$ is also
% a solution.
% \end{prop}
% \begin{proof}
% This i
% \end{proof}

\subsection{Algorithm}

Greedy search gives the optimal solution to the optimization (OPT) problem in
\ref{eq:cap_mimo}.





\begin{table}
\centering
\small{
    \begin{tabular}{|c|c||c|c|}
    \hline
    $B$ & 1000 B&  $Q_l$   &  2   \\
    \hline
    $\rho$  & 0dB  & $Q_h$ & 8   \\
    % \hline
    % $n$ & 8,16,32 & $D_i$  & 2$\mu$s \\
    \hline
    $m$ & 2  &  channel &  rayleigh \\
    \hline
    $\gamma(x)$ & $\frac{\pi\sqrt(3)}{2} 2^{-2x}$  &  $f_i$ & 20MHz \\
    \hline
    \end{tabular}
    }
\caption{MIMO simulation parameters}
\label{table:mimo_simu_params}
% \vspace{-15pt}
\end{table}
%

%
\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/sched_radio}
    \caption{Maximum rate as the link capacity is varied.\label{fig:sched_radio}}
\end{figure}
%

\subsection{Simulation Results}

We obtain the maximum wireless rate according to Eq.~\eqref{eq:cap_mimo} for a small-scale
simulated setup. Table~\ref{table:mimo_simu_params} shows the simulation parameters.
We consider a Rayleigh channel model, with two transmit antennas and SNR (without
quantization) of 0 dB. For ease of comparison, we set the deadlines of all flows
to be equal to their periods, i.e., $D_i = T_i$ for all $i \in \{1, \ldots, n\}$. We
use a rate monotonic scheduler as the fixed priority scheduler. Fig.~\ref{fig:sched_radio}
shows the maximum sum wireless rate averaged over channel realizations. Note that
as the link capacity $L$ increases, the transmission times decreases, thus the schedulability
supports higher quantization rates resulting in increased  throughput. For instance,
consider $n=8$, the rate increases (from 2-bit to 4-bit quantization) at 7Gbps,
and then further at 15Gbps (from 4-bit to 8-bit quantization). Also, as we increase
the number of radios from 8 to 32, we need at least 30Gbps aggregation link capacity
for the baseband packets to meet their deadlines.




% \end{theorem}

% \begin{proof}
% The proof is

% \end{proof}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% related %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Related Work}\label{related}


The concept of a Fat-Tree topology originated from the work on non-blocking switch networks.
It is now widely used in data-center for building scalable architectures\cite{alfaras}.
We propose a simple Fat-Tree with one aggregation link per switch; however, the design
can be generalized to multiple aggregation links and cross-links for improved
fault-tolerance. The only restriction being that one should be able to bound the
queuing time at each switch.

A large-scale MU-MIMO was realized using a distributed architecture
of servers in \cite{bigstation:13}. The authors claim that bandwidth needed for
baseband transport is not an issue as modern switches support up to 40Gbps links.
However, they do not consider the real-time guarantees of transporting
baseband samples. ARGOS\cite{argos} is another practical multi-antenna setup
that suggests daisy-chained radios with Tree-based aggregation. However, no
real-time analysis was provided.

Fronthaul transport using scheduled Ethernet design is used in \cite{ashwood}
to eliminate jitter. However, its design requires global scheduling.
On the other hand, \cite{spiro, uta} study the compression of baseband signals.
The authors propose different quantization schemes for lossy compression of the baseband samples.
In \cite{spiro}, the authors propose prioritization of baseband frames. However,
their method cannot provide any latency guarantees.

Real-time transport of Ethernet packets is a well-known problem in real-time systems
literature \cite{kandlur:91, hui:95, survey:94}. While \cite{kandlur:91} provides
a general approach for schedulability, the authors assume the use of flow regulators at
each switch according to logical arrival times, which is infeasible in practice.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% conclusion %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}\label{conclusion}

In this chapter, we design a baseband transport network that is scalable to a
large number of radios while meeting the end-to-end deadlines. We provide the
sufficient criteria for end-to-end schedulability,  which is validated in our
simulations. Our design can enable processing of wireless signals away from
hardware while ensuring no performance degradation from deadline misses.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Appendix}\label{appendix}


% link delay calculation: switch, propagation, transmission
\begin{theorem}\label{theorem:fixed}
Under fixed-priority scheduling, a set of traffic flows $\tau_i = (T_i, d_i), i = 1,2,\ldots, n$,
and priorities $\pi_i$, $i = 1,2,\ldots, n$,  such that $\pi_1 \geq \pi_2 \geq \ldots \geq \pi_n$, is schedulable
on a link with transmission time $C$, if the function $W_m (k,x)$ satisfies:
\begin{equation}
\max_{1\leq m\leq n} \max_{k \leq N_m} W_m (k, (k-1)T_m + d_m) \leq 1
\end{equation}
%
where $N_m = \min\{k : W_m(k, kT_m) \leq  1\}$, and function $W_m (k,x)$, for preemption, is defined as \cite{cmu:90}:
\begin{equation}
W_m(k,x) = \min_{0<t\leq x} \frac{C}{t}\left ( k+ \sum_{i=1}^{m-1} \left\lceil t/T_i\right\rceil \right),
\end{equation}
%
and without preemption, $W_m (k,x)$ is defined as \cite{utah:99}:
\begin{equation}
W_m(k,x) = \min_{0<t\leq x} \frac{C}{t}\left ( k+1 + \sum_{i=1}^{m-1}\left(1 + \left\lfloor{(t-C)/T_i}\right\rfloor \right) \right)
\end{equation}
%
\end{theorem}


\begin{theorem}\label{theorem:edf}
Under deadline scheduling, a set of traffic flows $\tau_i = (T_i, d_i), i = 1,2,\ldots, n$,
is schedulable on a link with transmission time $C$, and preemption if and only if \cite[Theorem 1]{cmu:90}:
\begin{equation}\label{eq:edf}
\forall t>0, \quad \frac{C}{t}\left(\sum_{i=1}^{n}\left\lceil{(t-d_i)/T_i}\right\rceil^{+}\right) \leq 1,
\end{equation}
%
and without preemption if and only if \cite[Theorem 6]{zheng:94}:
\begin{equation}
\forall t\geq d_{min}, \quad \frac{C}{t}\left(1 + \sum_{i=1}^{n}\left\lceil{(t-d_i)/T_i}\right\rceil^{+}\right) \leq 1
\end{equation}
%
where $d_{min} = \min\{d_i: 1\leq i \leq n\}$ and the function $\lceil x \rceil^{+} = max(0,\lceil x \rceil)$.
\end{theorem}
